On Self-Contact and Human Pose

People touch their face 23 times an hour, they cross their arms and legs, put their hands on their hips, etc. While many images of people contain some form of self-contact, current 3D human pose and shape (HPS) regression methods typically fail to estimate this contact. To address this, we develop new datasets and methods that significantly improve human pose estimation with self-contact. First, we create a dataset of 3D Contact Poses (3DCP) containing SMPL-X bodies fit to 3D scans as well as poses from AMASS, which we refine to ensure good contact. Second, we leverage this to create the Mimic-The-Pose (MTP) dataset of images, collected via Amazon Mechanical Turk, containing people mimicking the 3DCP poses with selfcontact. Third, we develop a novel HPS optimization method, SMPLify-XMC, that includes contact constraints and uses the known 3DCP body pose during fitting to create near ground-truth poses for MTP images. Fourth, for more image variety, we label a dataset of in-the-wild images with Discrete Self-Contact (DSC) information and use another new optimization method, SMPLify-DC, that exploits discrete contacts during pose optimization. Finally, we use our datasets during SPIN training to learn a new 3D human pose regressor, called TUCH (Towards Understanding Contact in Humans). We show that the new self-contact training data significantly improves 3D human pose estimates on withheld test data and existing datasets like 3DPW. Not only does our method improve results for self-contact poses, but it also improves accuracy for non-contact poses. The code and data are available for research purposes at https://tuch.is.tue.mpg.de.

==> main_sections/04_1_registeration.tex <==
\begin{figure}[t]
\includegraphics[width=\textwidth,height=5cm]{example-image-a}
\caption{Placehoder Figure highlighting }
\label{fig:contact}
\end{figure}
Raw 3D meshes  from a full body scanner have a variable number of vertices and the mesh topology is not consistent across different scans. We first process the raw scans into a structured format, that we refer to as a Registerations. The registerations are obtained by mapping the raw 3D scans to the template mesh of SMPL-X.  The mapping is achieved by iteratively deforming the template $V$ to minimize the \emph{point-to-plane} distance between the scan points $S \in \mathbb{R}^{N\times3}$, where $N$ is the number of scan points and the template points $V \in \mathbb{R}^{10375 \times 3}$.  \par 
More formally we follow the Co-Registeration algorithm by Hirshberg et al. \cite{Hirshberg:ECCV:2012} that we summarize below for the reader convenience. We define a data term $E_S$ evaluating the goodness of fit of the template  $V$ to the surface of the scan $S$. We randomly sample $N$ samples from the surface of the scan $x_s$ and minimize the data term between the scan samples $x_s$ and template verticies $x_v$ defined in equation \ref{eq:co_registeration}: 
\begin{equation}
\label{eq:co_registeration}
E_S( S;V) = \frac{1}{N} \int_{x_s \in \mathcal{S}} \rho \left( \left\lVert  x_s - x_v  \right\lVert \right)
\end{equation}
Where $\rho$ is a Geman-McClure robhustifier function \cite{}. The data term $E_S$ is minimized in two folds: first using the pose parameters $\vec{\theta} \in \mathbb{R}^{55\times3}$  and body shape parameters $\vec{\beta}\in\mathbb{R}^{25}$. Following a model-fit, then the template verticies $V$ are minimized to be close to the registeration.\par  
Registering poses with self-contact is challenging. When body parts are in close proximity, solely minimizing the data term $E_S$ results in interpentration, and implausiable deformation to the mesh template as shown in Figure \ref{fig:contact}. Our key insight is minimizing the data term is insufficient to preserve contact between body parts in close proximity, an additional contact term that minimize and perseve a \emph{point-to-plane} between body parts that are in contact is necessary. \par 
In addition to an energy term $E_S$ and contact-perserving loss term $E_C$ is minimized. On each optimization iteration, an indicator function $\mathbb{I_C}(x_v^{i};x_v^{j})$ is used to test whether to vertices $x_v^{i}$ and $x_v^{j}$ are in contact or not as follows:
\begin{equation}
  \mathbb{I_C}(x_v^{i};x_v^{j}) = 
  \begin{cases}
    1 & \text{if $G(x_v^i;x_v^j)>t_g$ and $E(x_v^i;x_v^j)<t_e $} \\
    0 & \text{otherwise}
  \end{cases}
\end{equation}
where $G(.;.)$ is the geodesic distance function, $t_g$ is a predifined threshold and $E(.;.)$ is the euclidean distance $t_e$ is a preddefined threshold in $mm$. Given the tuples of verticies $x_v^{i}$ and $x_v^{j}$ where  $\mathbb{I_C}(x_v^{i};x_v^{j})=1$, we minimize the \emph{point-to-plane} distance between $x_v^{i}$ and the triangular planes defined by $x_v^{j}$. In contrast to the \emph{point-to-point} distance, the \emph{point-to-plane} distance ensure that that body part remain on the surface of the template mesh defined by the template verticies and triangles. 
\begin{figure}[t]
\includegraphics[width=\textwidth,height=5cm]{example-image-a}
\caption{Placehoder Figure highlighting }
\label{fig:contact}
\end{figure}

Figure \ref{fig:contact} compares registerations with and without the contact term. Adding the contact term preserve the distance on the mesh surface


